A Stationary Mean-Field Model for Carbon Market Stability Reserve

We formulate the design of a market stability reserve as a stationary mean-field singular control problem. The allowance balance follows a regime-switching diffusion, while the regulator injects or withdraws allowances through bounded-variation controls. The objective trades off the average allowance balance, its stationary dispersion, deviations from a long-run target, and intervention costs. The optimal policy is a regime-dependent band rule characterized by four reflecting thresholds. Its computation reduces to a scalar fixed-point problem combining a coupled variational inequality with the invariant distribution of the reflected process. A calibration to the EU ETS yields thresholds of the same order of magnitude as the existing Market Stability Reserve rule. Comparative statics show that volatility is the main determinant of the intervention band, whereas the frequency and duration of crisis regimes have limited effects. A simpler two-threshold policy based on average regime dynamics closely reproduces the optimal regime-dependent policy in terms of liquidity and intervention volumes.

==> policy_intervention_table_V2.tex <==
\begin{table}[!hbt]
\centering
\small
\begin{tabular}{cccccccc}
\hline
$\delta_2$ & $\pi_2$ & $I_+^*$ & $I_+^{\mathrm{av}}$ & $\Delta I_+/I_+^*$ (\%) & $I_-^*$ & $I_-^{\mathrm{av}}$ & $\Delta I_-/I_-^*$ (\%) \\
\hline
0.000 & 0.010 & 250 & 250 & 0.06 & 212 & 211 & -0.24 \\
0.020 & 0.010 & 250 & 250 & 0.07 & 212 & 211 & -0.23 \\
0.040 & 0.010 & 250 & 250 & 0.07 & 211 & 211 & -0.23 \\
0.060 & 0.010 & 250 & 250 & 0.07 & 211 & 211 & -0.23 \\
\hline
0.000 & 0.094 & 249 & 249 & -0.02 & 214 & 213 & -0.31 \\
0.020 & 0.094 & 249 & 249 & 0.07 & 213 & 212 & -0.22 \\
0.040 & 0.094 & 249 & 250 & 0.07 & 212 & 212 & -0.23 \\
0.060 & 0.094 & 250 & 250 & 0.07 & 212 & 211 & -0.23 \\
\hline
0.000 & 0.200 & 247 & 247 & -0.17 & 216 & 215 & -0.51 \\
0.020 & 0.200 & 248 & 248 & 0.02 & 215 & 214 & -0.33 \\
0.040 & 0.200 & 249 & 249 & 0.02 & 214 & 213 & -0.36 \\
0.060 & 0.200 & 249 & 249 & 0.01 & 212 & 212 & -0.37 \\
\hline
\end{tabular}
\caption{Long-run intervention intensities under the optimal regime-dependent policy and under the policy obtained from the averaged one-regime model, both evaluated under the true two-regime dynamics. Intervention intensities are reported in Mt/year.}
\label{tab:policy_interventions}
\end{table}


==> policy_liquidity_table_V2.tex <==
\begin{table}[!hbt]
\centering
\small
\begin{tabular}{ccccc}
\hline
$\delta_2$ & $\pi_2$ & $L^*$ (Mt) & $L^{\mathrm{av}}$ (Mt) & $\Delta L/L^*$ (\%) \\
\hline
0.000 & 0.010 & 69 & 69 & -0.05 \\
0.020 & 0.010 & 69 & 69 & -0.04 \\
0.040 & 0.010 & 69 & 69 & -0.04 \\
0.060 & 0.010 & 69 & 69 & 0.00 \\
\hline
0.000 & 0.094 & 69 & 69 & -0.43 \\
0.020 & 0.094 & 69 & 69 & -0.34 \\
0.040 & 0.094 & 69 & 69 & -0.34 \\
0.060 & 0.094 & 69 & 69 & 0.00 \\
\hline
0.000 & 0.200 & 69 & 68 & -1.76 \\
0.020 & 0.200 & 69 & 68 & -1.57 \\
0.040 & 0.200 & 69 & 68 & -1.57 \\
0.060 & 0.200 & 69 & 68 & -0.84 \\
\hline
\end{tabular}
\caption{Stationary liquidity shortfall under the optimal regime-dependent policy and under the policy obtained from the averaged one-regime model, both evaluated under the true two-regime dynamics. Here $L(A)=\mathbb{E}[(\bar\theta-X)^+]$ and $\Delta L/L^*=(L^{\mathrm{av}}-L^*)/L^*$.}
\label{tab:policy_liquidity}
\end{table}

